Encouraging Diversity- and Representation-Awareness in Geographically Centralized Content

In centralized countries, not only population, media and economic power are concentrated, but people give more attention to central locations. While this is not inherently bad, this behavior extends to micro-blogging platforms: central locations get more attention in terms of information flow. In this paper we study the effects of an information filtering algorithm that decentralizes content in such platforms. Particularly, we find that users from non-central locations were not able to identify the geographical diversity on timelines generated by the algorithm, which were diverse by construction. To make users see the inherent diversity, we define a design rationale to approach this problem, focused on an already known visualization technique: treemaps. Using interaction data from an "in the wild" deployment of our proposed system, we find that, even though there are effects of centralization in exploratory user behavior, the treemap was able to make users see the inherent geographical diversity of timelines, and engage with user generated content. With these results in mind, we propose practical actions for micro-blogging platforms to account for the differences and biased behavior induced by centralization.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
last modified by Bernhard Finkbeiner, July 5, 2010

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored by
the IEEE Visualization & Graphics Technical Committee (VGTC).

The only conferences that use the 'journal' document option:
- IEEE Visualization Conference (Research and Application Papers Only)
- IEEE Information Visualization Conference (Research and Application
Papers Only)

It contains 13 files:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed,
                  somewhere in the TeX search path
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
sample.eps      - an image used by the example paper
sample.pdf      - its PDF version
template-journal*.pdf    - an example proper pdf output in default
                          conference mode, with and without teaser
CypressView.eps - teaser image
CypressView.pdf - its PDF version
makefile     - makefile including bibtex compilation and proper PDF
                generation

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We
suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create
a file called 'template.pdf'. Please make sure, that its layout is
identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process
manually.  Below are a list of available options that may be passed to
make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> discussion.tex <==
% THIS FILE IS NOT IN THE PAPER ANYMORE (IT WILL BE REINSTATED ON THE THESIS)

We now discuss two important implications of our results.

\spara{Importance of Social Contexts}
It is expected that different cultures and societies have different behaviors in both off- and on-line worlds.
Anything that influences those social contexts is likely to also influence behavior, as geographical centralization does.
In this work, we show that in a centralized country \textit{people do not only behave differently, but they also understand information differently} depending on whether they live in a central, over-represented location or not. 
Therefore, individual differences are not bound by personality traits, demographic factors or ad-hoc expertise for the task at hand. 
The social and physical context also defines an individual difference which should be considered when designing algorithms and user interfaces, because in a globalized world a \emph{``one-size-fits-all''} approach is likely to ignore cultural and behavioral differences.

\spara{A Better Algorithm is Not Enough}
When designing algorithms, it is important to account explicitly for the behavior that we want to ``enhance'', but algorithms by themselves are not enough.
In our case, even though the algorithm described in Section \ref{sec:algorithm} presented a balanced and diverse timeline, it was not enough for users to \emph{see} that diversity and thus, to feel represented. A change of user interface was needed.
Extending design guidelines from previous literature, we designed a user interface that surfaced how differently people behave based on their location by employing the \textit{treemap} visualization technique. 
Since users, regardless of their location, explored more locations and spent more time on the site using our design, we can conclude that the right mix of information filtering plus interface design helps to make users aware of the diverse locations represented.
How to transform this awareness into value for users is a challenge for future work.

% A NICE QUOTE WOULD BE GOOD HERE?
% Still thinking on what to do here...

==> methodology.tex <==
We briefly explain the algorithm used to generate the diversified timelines. This algorithm is used to carry out our experiments and was inspired from \cite{de2011identifying,munson2009sidelines}.
Given a set of microposts $T_{E}$, the algorithm generates a filtered tweet set $T_{\theta}$, where $T_{\theta}$ contains $s$ tweets and $s \leq |T_{E}|$;
and $T_{\theta}$ is geographically diverse, i.e. $\text{geodiversity}(T_{\theta}) \geq \text{geodiversity}(T_{E})$. 

\spara{Geographical Diversity}
We define geographical diversity as the normalized \emph{Shannon entropy} \cite{jost2006entropy} with respect to a set of locations $L$ (where $|L| > 1$):
\[\text{geodiversity} = \frac{-\sum_{i = 1}^{|L|} p_{i} \ \ln {p_{i}}}{\ln |L|}\]
where $p_{i}$ is the probability that a micropost is related to a location $\ell_i$. Geodiversity is $0$ when all microposts are from one location only, and geodiversity is $1$ when all locations are represented equally.

\spara{Input Features}
For each micropost $t$, we consider a vector representation $\vec{v_{t}}$ with the following features:

\begin{enumerate}
  \item \emph{Presence of links}: whether the micropost contains a URL or not.
  \item \emph{Time bucket}: time passed since the start of $E$.
  \item \emph{Annotated hashtags}: topical information.
  \item \emph{Geography}: defined as the location its content is most likely to be about.
  \item Author's number of \emph{followers}.
  \item Author's \emph{hub dimension} ($\frac{\text{followers}}{\text{friends}}$).
  \item Author's \emph{global micropost count}.
  \item \emph{Popularity}: number of times it has been republished by others.
\end{enumerate}

All features are bucketed. We consider buckets based on the logarithms of each value when applicable.
%In \cite{de2011identifying} popularity was not a feature. It was not needed,  as tweet selection was made in the context of a previously filtered set in relation to given topics (for instance, \textit{oil spill}).
%It is assumed that filtering of those tweets selected content relevant enough to be considered, while our context is more general and thus we need to have some notion of relevance.
%We chose to consider popularity, as it has been established as a valuable feature for tweet recommendation \cite{chen2010short,chen2012collaborative}. 

% \spara{Location \textit{Sidelines}}
% Since the complexity of feature dimensions can be greater than those of geography (for instance, consider the number of hashtags in an event against the number of locations), the entropy contribution of these dimensions can be higher than the entropy contribution of geography.
% Thus, geographical diversity needs to be enforced by adding a \textit{sidelining} step \cite{munson2009sidelines} when considering tweets for selection, i.e. tweets from a location previously selected in the previous iterations of the algorithm will not be considered during a given number of $n$ turns.
% %Thus, diversity could still be optimal in the absence of geographical diversity.
% %And, given that popularity is likely linked to population imbalance (i.e., tweets from more populated locations are likely to be more popular than those from less populated locations, an imbalance strengthened by centralization), we need to enforce geographical diversity by adding a \textit{sidelining} step \cite{munson2009sidelines} when considering tweets for selection, i.e. tweets from a location previously selected in the previous iterations of the algorithm will not be considered during a given number of $t$ turns.

\spara{Algorithm Definition}
%Given a set of tweets $T_{E}$, we generate a filtered tweet set $T_{\theta}$, where $T_{\theta}$ contains $s$ tweets.
To maximize geographical diversity in $T_{\theta}$, we consider a greedy algorithm:
start by randomly selecting a micropost $t$ from the most popular bucket from $T_{E}$ as initial seed in $T_{\theta}$.
Then, greedily increment $T_{\theta}$ by adding a selected micropost from $T_{E}$. 
To select this micropost, build a candidate set $T_{c}$ where every micropost $t$ satisfies the following: 
\begin{enumerate}
  \item It has not been already added, i.e., it is not in $T_{\theta}$.
  \item Its addition to $T_{\theta}$ maximizes information entropy \cite{jost2006entropy} $H_{\theta} = -\sum_{i = 1}^{k} p(\vec{v_{t_{i}}}) \ln p(\vec{v_{t_{i}}})$.
  \item Its location has not been considered before in at least $n$ turns \cite{munson2009sidelines}.
  \item It terms of popularity, it is on the most popular bucket.
\end{enumerate}
Repeat until $|T_{\theta}| = s$. 

The algorithm is shown in pseudo-code in Algorithm \ref{alg:filtering_timeline}.
It was evaluated in \cite{graellsbalancing}, and was found to be more geographically diverse than its base algorithm \cite{de2011identifying}, and that a popularity-based timeline from a centralized country was not geographically diverse at all, as geodiversity was close to $0$.
In the next sections we evaluate how this algorithm performs considering user-centered attributes.

\begin{algorithm}[tbp]
\caption{Geo. Diverse Information Filtering Algorithm.}
\label{alg:filtering_timeline}
\scriptsize
\begin{algorithmic}
\Require $T \gets \text{set of microposts to be filtered}$
\Require $s \gets \text{cardinality of resulting filtered set}$
\Require $\text{turns} \gets \text{number of turns for sidelining}$
\Ensure $T_{\theta} \gets \text{filtered micropost set}$

\Function{$\text{geodiverse\_filtering}$}{$(T, s, \text{turns})$}
\State $T_{\theta} \gets \text{list()}$
\State $\text{sidelined} \gets \text{dictionary}()$
\ForAll{$\ell \text{ in } L$}  
   \State $\text{sidelined}[\ell] \gets 0$
\EndFor

\State $t \gets \text{random.choice}(\text{most\_popular\_microposts}(T_{E}))$
\State $T_{\theta}.\text{append}(t)$
\State $\text{sidelined}[t_{\ell}] \gets \text{turns}$

\Repeat  
  \State $T_{c} \gets \text{list()}$
  \ForAll{$t \text{ in } T_{E} \text{ not in } T_{\theta}$}  
      \If{$\text{max\_entr}(t, T_{\theta}) \text{ and } \text{sidelined}[t_{\ell}] \leq 0$}
          \State $T_{c}.\text{append}(t)$
      \EndIf
   \EndFor
   
   \State $t \gets \text{random.choice}(\text{popular\_microposts}(T_{c}))$
   
   \State $T_{\theta}.\text{append}(t)$
   \State $\text{sidelined}[t_{\ell}] \gets \text{turns} + 1$
   
   \ForAll{$\ell \text{ in } L$}  
      \State $\text{sidelined}[\ell] \gets \text{sidelined}[\ell] - 1$
      
   \EndFor
\Until{$|T_{\theta}| = s$}
\State \Return $T_{\theta}$
\EndFunction
\end{algorithmic}
\end{algorithm}
